TIARA: Multi-grained Retrieval for Robust Question Answering over Large Knowledge Bases

Pre-trained language models (PLMs) have shown their effectiveness in multiple scenarios. However, KBQA remains challenging, especially regarding coverage and generalization settings. This is due to two main factors: i) understanding the semantics of both questions and relevant knowledge from the KB; ii) generating executable logical forms with both semantic and syntactic correctness. In this paper, we present a new KBQA model, TIARA, which addresses those issues by applying multi-grained retrieval to help the PLM focus on the most relevant KB contexts, viz., entities, exemplary logical forms, and schema items. Moreover, constrained decoding is used to control the output space and reduce generation errors. Experiments over important benchmarks demonstrate the effectiveness of our approach. TIARA outperforms previous SOTA, including those using PLMs or oracle entity annotations, by at least 4.1 and 1.1 F1 points on GrailQA and WebQuestionsSP, respectively.

==> emnlp2021_0527.tex <==

% background
Knowledge bases (KB) maintain abundant reliable real-world facts in a structured form.
However, it is not easy to query the KBs with daily unstructured natural language.
Question Answering over Knowledge Base (KBQA) attempts to provide a user-friendly way to query KB facts.
%%Knowledge bases (KB) contain abundant world facts curated by human in a structured form, which can be easily controlled or updated. However, people can not directly ask questions and obtain the expected answers in KBs. Question Answering over Knowledge Base (KBQA) attempts to solve the problem and provides a user-friendly way for users to query KB facts. 

% challenges
The KBQA task requires adequate question understanding and KB retrieval and reasoning capabilities.
Existing approaches are mainly divided into two categories, i.e., information retrieval-based (IR-based) methods and semantic parsing-based (SP-based) methods \cite{lan21asurvey}.
IR-based methods \cite{shi21transfer,zhang22subgraph} retrieve subgraphs and rank paths from the topic entity to the answer without requiring SPARQL annotations, but their reasoning processes are difficult to interpret.
In contrast, SP-based methods map unstructured natural language questions to interpretable logical forms (e.g., query graph \cite{yih15semantic}, S-expression \cite{gu21beyond}), and then convert them into executable queries.
% Logical forms support complex reasoning, and generating logical forms requires query composition in addition to retrieving entities and schema.
% There is a huge gap in syntactic and semantic diversity between natural language and logical forms.
According to the logical form generation manners, they can be divided into query-graph generation methods and transduction-based methods.
\textit{Query-graph generation methods} \cite{yih15semantic,lan20query} iteratively expand the query graph and the process follows a strict syntax.
However, it can only start searching from entities and is limited to a fixed number of hops\footnote{Since the search space grows exponentially with the number of hops, it is usually 2-3 hops.} due to efficiency.
But the question may either not contain an entity or may go beyond the two-hop range.
Also, due to the huge combinatorial space, it is difficult to enumerate all the functions (e.g., COUNT, ARGMAX, ARGMIN) supported by the logical form when searching on the KB.
\textit{Transduction-based methods} translate natural language questions to logical forms in a sequence-to-sequence manner.
It is not limited to the existence of entities, the number of hops or functions, compared to the query-graph generation methods described above.
In particular, Pre-trained Language Models (PLMs) have shown state-of-the-art generation capabilities.
However, they are pre-trained on the natural language and may not adequately learn the syntax and semantics of the logical forms when fine-tuned on the KBQA task.
It brings two challenges: 1) how to make PLMs associate natural language to relevant KB entities, schema or reasoning paths, 
and 2) how to make the generated logical forms conform to the syntactic constraints.

First, our pilot experiments show that given the question with oracle entities, schema, and candidate logical forms, T5-base \cite{raffel2022exploring} can achieve up to 92.4\% F1 on the GrailQA \cite{gu21beyond} validation set.
It shows that PLM works well in query composition given the correct KB context.
Improving the retrieval of entities, schema, and logical forms becomes the key to leveraging PLM generation capabilities.
\citet{chen21retrack} retrieve hundreds of KB schema for generation, with an excessive number of schema candidates and poor zero-shot generalization performance.
\citet{das21case} retrieve similar questions with query annotations in the training set.
However, it only conforms to the i.i.d. assumption.
\citet{zan22s2ql} also propose a retrieval method on the training set.
\citet{ye21rng} enumerate and rank candidate logical forms before the generation in a query-graph search method with drawbacks described above.
Therefore, we consider multi-grained retrieval to cope with the inadequacy of retrieving only schema or logical forms.
Also, the retrieval is performed on the KB instead of any dataset with query annotation to cope with compositional and zero-shot generalization scenarios.
Experiments show that the retrieved schema and candidate logical forms complement each other and help PLM generate more flexible logical forms.

Secondly, in the absence of using pre-trained Seq2Seq models, transduction-based methods NSM \cite{liang17neural} and ReTraCk \cite{chen21retrack} use syntax rules to ensure generated logical forms are syntactically correct.
Compared to them, the decoding space of PLMs is not limited and it is prone to generating invalid logical forms.
Inspired by constrained decoding methods for other semantic parsing tasks such as text2SQL \cite{picard21scholak}, we introduce constrained decoding to PLM on the KBQA task for the first time.
It better guides PLM to generate logical forms without additional training or retrieval, reducing common generation errors.

% Due to the large size of the KB and the difficulty of obtaining annotated data, the model can only see a part of the schema (i.e., class and relation) of the KB.
% It requires the model to have the ability to handle questions for compositional and zero-shot generalization \cite{keysers20measuring,gu21beyond}.

% contributions
The contributions are as follows.
\begin{itemize}
    \item To exploit the generation capabilities of PLMs on KBQA task, we investigate mul\textbf{TI}-gr\textbf{A}ined \textbf{R}etrieval-\textbf{A}ugmentation (\textbf{TIARA}) methods including entity linking, logical form retrieval, and schema retrieval.
    \item Experiments demonstrate that our method not only achieves state-of-the-art performance on the i.i.d. WebQSP dataset, but also shows better generalization abilities than existing methods on GrailQA dataset.
\end{itemize}


\section{Related Work}
% Moreover, it assumes the search starts with an entity, but the question may not even be associated with any KB entity.
% Even so, it could generate logical forms with a limited number of hops, providing context for augmenting the transduction-based methods \cite{ye21rng}.

% Logical forms may have complex compositionality and the generation needs to follow syntactic requirements.
% \citet{liang17neural} handle the query compositionality with a key-variable memory and prune the search space with a Lisp interpreter.
% \citet{chen21retrack} first retrieve KB items, then follow syntax rules to generate queries and check the generated results statically and dynamically.


% PLMs have shown powerful text-to-text generation capabilities.
% Existing works use different retrieval methods to augment PLMs to generate logical forms.
% \citet{das21case} retrieve questions similar to the input question and use their query annotations, but it can only work by adding matching cases in a zero-shot scenario.
% \citet{ye21rng} iteratively rank candidate logical forms of the anchor entities within two hops.
% However, logical forms are not always available due to the absence of entities and the limited number of hops.
% \citet{xie22unified} retrieve KB schema related to the question.
% Though transduction-based methods with PLMs have achieved state-of-the-art performance, their lack of syntax rules easily leads to invalid logical forms.
% To address the above issues, this paper focuses on the methods of retrieval augmentation and decoding constraints of PLMs.
